Answering Complex Questions by Joining Multi-Document Evidence with Quasi Knowledge Graphs

Direct answering of questions that involve multiple entities and relations is a challenge for text-based QA. This problem is most pronounced when answers can be found only by joining evidence from multiple documents. Curated knowledge graphs (KGs) may yield good answers, but are limited by their inherent incompleteness and potential staleness. This paper presents QUEST, a method that can answer complex questions directly from textual sources on-the-fly, by computing similarity joins over partial results from different documents. Our method is completely unsupervised, avoiding training-data bottlenecks and being able to cope with rapidly evolving ad hoc topics and formulation style in user questions. QUEST builds a noisy quasi KG with node and edge weights, consisting of dynamically retrieved entity names and relational phrases. It augments this graph with types and semantic alignments, and computes the best answers by an algorithm for Group Steiner Trees. We evaluate QUEST on benchmarks of complex questions, and show that it substantially outperforms state-of-the-art baselines.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> fig-example-sentence.tex <==
\newcommand{\smlnumber}[1]{${}^{#1}$}
\begin{quote}\it%
%\smlnumber{0}%
Didier Yves Drogba T\'{e}bily 
%\smlnumber{5}%
born 
%\smlnumber{6}%
(11 March 1978)
%\smlnumber{10}%
is 
%\smlnumber{11}%
an 
%\smlnumber{12}%
Ivorian 
%\smlnumber{13}%
professional footballer 
%\smlnumber{15}%
who
%\smlnumber{16}%
plays 
%\smlnumber{17}%
as 
%\smlnumber{18}%
a 
%\smlnumber{19}%
striker
%\smlnumber{20}%
for
%\smlnumber{21}%
American 
%\smlnumber{22}%
club 
%\smlnumber{23}%
Phoenix Rising. 
\end{quote}


==> tbl-analysis.tex <==
\begin{table*} [t]
	\begin{tabular}{l c c l c c}
		\toprule
		\textbf{Graph configuration}	&	\textbf{CQ-150}			&	\textbf{TQ-100}			& \textbf{Answer ranking criterion}		&	\textbf{CQ-150}			&	\textbf{TQ-100}			& \textbf{Error scenario}								&	\textbf{CQ-150}	&	\textbf{TQ-100}	\\ \toprule 
		Full configuration				&	$\boldsymbol{0.314}$	&	$\boldsymbol{0.351}$	& Sum of node weights						&	$\boldsymbol{0.315}$	&	$\boldsymbol{0.351}$	& Answer not in initial corpus						&	$13\%$				&	$11\%$				\\ 
		No types						&	$0.153$*				&	$0.107$*				& Number of GSTs ($k$)					&	$0.314$					&	$0.347$	& Answer in initial corpus but absent in quasi KG		&	$43\%$				&	$28\%$				\\
		Degenerate edge weights			&	$0.269$*				&	$0.264$*				& Sum of inverses of tree costs			&	$0.306$					&	$0.344$					& Answer in quasi KG but absent in top-$50$ GSTs		&	$17\%$				&	$27\%$				\\ 
		No alignment edges				&	$0.302$					&	$0.319$*				& Weighted distance to all cornerstones	&	$0.252$*				&	$0.281$*				& Answer in top-$50$ GSTs but not in candidates		&	$14\%$				&	$30\%$				\\
		No entity alignment edges		&	$0.312$					&	$0.297$					& Unweighted distance to all cornerstones	&	$0.270$*				&	$0.291$*			& Answer in candidates but not in top-$5$				&	$13\%$				&	$4\%$				\\ \bottomrule
		% No predicate alignment edges	&	$0.308$					&	$0.355$	\\ \bottomrule		
	\end{tabular}
	\label{tab:analysis}
\end{table*}


%----
\begin{table} [t]
	\small
\input{tbl-graph-ablation.tex}
	\mycaption{Graph ablation studies for {\quest} with {\MRRatk{5}}
	on top-$10$ corpora.
	 The highest value per column is marked in \textbf{bold}. 
	 % rishi: removing article ('a') for '*', should be 'an' for asterisk.
	 ``$*$'' denotes statistically significant difference w.r.t.
	 the full configuration.}
  \label{tab:ablation}
  \vspace*{-0.7cm}
\end{table}
%----

==> tbl-corpus-comparisons.tex <==
\begin{tabular}{l c c c c}
	\toprule
	\textbf{Corpus}	& \textbf{Web}	& \textbf{News} & \textbf{Wiki} & \textbf{All}	\\ \toprule
	Wiki-$150$		& $0.513$		& $0.480$*		& $0.380$*		& $0.513$ 		\\
	Trends-$150$	& $0.349$*		& $0.400$		& $0.213$*		& $0.427$		\\ \bottomrule
\end{tabular}

==> tbl-errors.tex <==
\begin{tabular}{l c c}
	\toprule
	\textbf{Error scenario}								&	\textbf{CQ-150}	&	\textbf{TQ-100}	\\ \toprule
	Answer not in initial corpus						&	$13\%$				&	$11\%$				\\ 
	Answer in initial corpus but absent in quasi KG		&	$43\%$				&	$28\%$				\\
	Answer in quasi KG but absent in top-$50$ GSTs		&	$17\%$				&	$27\%$				\\
	Answer in top-$50$ GSTs but not in candidates		&	$14\%$				&	$30\%$				\\
	Answer in candidates but not in top-$5$				&	$13\%$				&	$4\%$				\\ \bottomrule		
\end{tabular}


==> tbl-graph-ablation.tex <==
\begin{tabular}{l c c}
	\toprule
	\textbf{Graph configuration}	&	\textbf{CQ-150}			&	\textbf{TQ-100}	\\ \toprule
	Full configuration				&	$\boldsymbol{0.314}$	&	$\boldsymbol{0.351}$	\\ \midrule
	No types						&	$0.153$*				&	$0.107$*	\\
	Degenerate edge weights			&	$0.269$*				&	$0.264$*	\\
	No alignment edges				&	$0.302$					&	$0.319$*	\\ \bottomrule
	% No entity alignment edges		&	$0.312$					&	$0.297$	\\
	% No predicate alignment edges	&	$0.308$					&	$0.355$	\\ \bottomrule		
\end{tabular}

==> tbl-graph-systems-strat.tex <==
\setlength{\tabcolsep}{0.8ex}
\begin{tabular}{l p{0.1ex} ccc ccc ccc ccc ccc ccc}			\toprule
	\multirow{2}{*}{\textbf{Method}}
	&	\multirow{2}{*}{$r$}
	&& 	\multicolumn{4}{c}{\textbf{CQ-150}}			
	&&	\multicolumn{4}{c}{\textbf{TQ-150}} 
	\cmidrule{4-7} \cmidrule{9-12}
	&
	&& 	\textbf{Top-10}			& \textbf{Strata-10-1}
	& 	\textbf{Strata-10-2}	& \textbf{Strata-10-3}
	&& 	\textbf{Top-10}	& \textbf{Strata-10-1}
	&& 	\textbf{Strata-10-2}	& \textbf{Strata-10-3}
\\ \midrule
	\quest					
	& 	$1$	
	&&	$\boldsymbol{0.267}$*	& $\boldsymbol{0.240}$*
	& 							& \\	
	\method{DrQA}~\cite{chen2017reading}					
	& 	$1$	
	&& 	$0.193$					& $0.160$
	& 							& 					\\	
	\bfs~\cite{kasneci2009star}					
	& $1$													\\	
	\shortestPath		
	& $1$													\\	\midrule
	\quest					
	& $3$	
	&& $\boldsymbol{0.307}$*	& $\boldsymbol{0.312}$*
	&& 							&
\\
	\method{DrQA}~\cite{chen2017reading}					
	& $3$	
	&& $0.238$					& $0.212$ 
	&& 							&
	&& $0.224$ 					& $\boldsymbol{0.218}$ 
	&&							&
	&& $\boldsymbol{0.243}$ 	& $\boldsymbol{0.253}$
	&& 							& \\	
	\bfs~\cite{kasneci2009star}				
	& $3$													\\
	\shortestPath		
	& $3$													\\	\midrule
	\quest					
	& $5$	
	&& $\boldsymbol{0.314}$*	& $\boldsymbol{0.317}$*
	&&							& 		
	&& $\boldsymbol{0.255}$*	& $0.215$ 
	&&							& 
	&& $0.222$					& $0.219$
	&&							& 							\\
	\method{DrQA}~\cite{chen2017reading}					
	& $5$	
	&& $0.248$					& $0.222$ 
	&&							& 
	&& $0.237$					& $\boldsymbol{0.227}$	
	&&							& 
	&& $\boldsymbol{0.243}$ 	& $\boldsymbol{0.255}$ 		\\
	\bfs~\cite{kasneci2009star}		
	& $5$													\\
	\shortestPath				
	& $5$													\\	\bottomrule
\end{tabular}

==> tbl-main-result.tex <==
% !TEX root = ../2018-cikm-fp-compqa-text.tex
%----suggest to use \multirow{3}for \quest and \bfs, and add another column 
%called "r", 
%\setlength{\tabcolsep}{1ex}
	%\begin{tabular}{p{3.5cm} c ccc}
	% rishi: full-300 should come first
	% confusing for reader to understand rank in same table
	% may accuse us of being opportunistic
	\begin{tabular}{l c c c}
		\toprule
		\textbf{Method} 								& \textbf{Full-300} 			& \textbf{Wiki-150} 		& \textbf{Trends-150}	 		\\ \midrule
%		\multirow{1}{*}{\quest} 						& $0.253$*						& $0.260$* 					& $0.247^\dagger$* 				\\
%														& $0.357$*						& $0.387$* 					& $0.327^\dagger$* 				\\
		{\quest}										& $\boldsymbol{0.470}$*			& $\boldsymbol{0.513}$* 	& $\boldsymbol{0.427}$ 			\\ \midrule
%		{\quest}										& $\boldsymbol{0.390}$*			& $\boldsymbol{0.427}$ 		& $\boldsymbol{0.353}$* 		\\ \midrule
%														& $\boldsymbol{0.487}$ 			& $\boldsymbol{0.547}$ 		& $\boldsymbol{0.427}$ 			\\ \midrule
%		\multirow{3}{*}{\bfs~\cite{kasneci2009star}}	$0.157$ 						& $0.147$ 					& $0.167$ 				 		\\
%														$0.293$ 						& $0.280$ 					& $0.307$ 				 		\\
		\method{DrQA}~\cite{chen2017reading}			& $\boldsymbol{0.433}$ 			& $0.373$ 					& $\boldsymbol{0.493}$ 			\\ \midrule				
		{\bfs~\cite{kasneci2009star}}					& $\boldsymbol{0.380}$ 			& $0.400$ 					& $\boldsymbol{0.360}$ 			\\ \midrule
%		\multirow{3}{*}{\shortestPath}					& $0.120$ 						& $0.107$ 					& $0.133$ 				 		\\
%														& $0.190$ 						& $0.160$ 					& $0.220$ 				 		\\
		{\shortestPath}									& $0.207$ 						& $0.180$ 					& $0.233$ 						\\ \midrule
		\paralex~\cite{fader2013paraphrase}				& $0.003$ 						& $0.007$ 					& $0.000$ 				 		\\
		% \paralex+\autoJoin							& $0.007$ 						& $0.013$ 					& $0.000$ 				 		\\
		\paralex+\manJoin								& $0.007$ 						& $0.013$ 					& $0.000$ 						\\
		% \paralex+\autoUnion							& $0.053$ 						& $0.100$ 					& $0.007$ 				 		\\
		\paralex+\manUnion								& $0.080$ 						& $0.153$ 					& $0.007$ 					 	\\ \midrule
		\aqqu~\cite{bast2015more}	 					& $0.133$ 						& $0.127$ 					& $0.140$ 				 		\\ 
		% \aqqu+\autoJoin								& $0.123$ 						& $0.107$ 					& $0.140$ 				 		\\
		\aqqu+\manJoin									& $0.263$ 						& $\boldsymbol{0.507}$ 		& $0.020$ 				 		\\
		% \aqqu+\autoUnion								& $0.210$ 						& $0.320$ 					& $0.100$ 				 		\\
		\aqqu+\manUnion									& $0.347$ 						& $\boldsymbol{0.573}$ 		& $0.120$ 				 		\\ \bottomrule				
	\end{tabular}
	
	
%	\begin{tabular}{l c c c c}
%		\toprule
%		\textbf{Method} 								& \textbf{Rank $r$}	& \textbf{Full-300} 			& \textbf{Wiki-150} 		& \textbf{Trends-150}	 		\\ \midrule
%%		\multirow{1}{*}{\quest} 						& $1$ 				& $0.253$*						& $0.260$* 					& $0.247^\dagger$* 				\\
%%														& $3$  				& $0.357$*						& $0.387$* 					& $0.327^\dagger$* 				\\
%		{\quest}										& $5$ 				& $\boldsymbol{0.390}^\dagger$ 	& $0.427$ 					& $\boldsymbol{0.353}^\dagger$ 	\\
%%														& All$^\blacktriangle$ 		& $\boldsymbol{0.487}$ 			& $\boldsymbol{0.547}$ 		& $\boldsymbol{0.427}$ 			\\ \midrule
%%		\multirow{3}{*}{\bfs~\cite{kasneci2009star}}	& $1$ 				& $0.157$ 						& $0.147$ 					& $0.167$ 				 		\\
%%														& $3$ 				& $0.293$ 						& $0.280$ 					& $0.307$ 				 		\\
%		{\bfs}											& $5$ 				& $\boldsymbol{0.380}$ 			& $0.400$ 					& $\boldsymbol{0.360}$ 			\\ \midrule
%%		\multirow{3}{*}{\shortestPath}					& $1$ 				& $0.120$ 						& $0.107$ 					& $0.133$ 				 		\\
%%														& $3$ 				& $0.190$ 						& $0.160$ 					& $0.220$ 				 		\\
%		{\shortestPath}									& $5$ 				& $0.207$ 						& $0.180$ 					& $0.233$ 					 	\\ \midrule
%		\paralex~\cite{fader2013paraphrase}				& -					& $0.003$ 						& $0.007$ 					& $0.000$ 				 		\\
%		\paralex+\autoJoin								& - 				& $0.007$ 						& $0.013$ 					& $0.000$ 				 		\\
%		\paralex+\manJoin								& -					& $0.007$ 						& $0.013$ 					& $0.000$ 						\\
%		\paralex+\autoUnion								& -					& $0.053$ 						& $0.100$ 					& $0.007$ 				 		\\
%		\paralex+\manUnion								& -			 		& $0.080$ 						& $0.153$ 					& $0.007$ 					 	\\ \midrule
%		\aqqu~\cite{bast2015more}	 					& - 				& $0.133$ 						& $0.127$ 					& $0.140$ 				 		\\ 
%		\aqqu+\autoJoin									& -			 		& $0.123$ 						& $0.107$ 					& $0.140$ 				 		\\
%		\aqqu+\manJoin									& - 				& $0.263$ 						& $\boldsymbol{0.507}$ 		& $0.020$ 				 		\\
%		\aqqu+\autoUnion								& -		 			& $0.210$ 						& $0.320$ 					& $0.100$ 				 		\\
%		\aqqu+\manUnion									& - 				& $0.347$ 						& $\boldsymbol{0.573}$ 		& $0.120$ 				 		\\ \bottomrule
%	\end{tabular}	

%    \begin{tabular}{l c c c}
%       \toprule
%       \textbf{Method}			& \textbf{---300} 	
%       		& \textbf{Wiki-150}			
%       			& \textbf{Trends-150}	\\ 
%       \toprule
%      {\questat{1}}							
%      	& $0.267$				
%      		& $0.000$
%      							& $0.000$	\\
%       {\questat{3}}							& $0.440$				& $0.000$					& 
%$0.000$	\\ 
%       {\questat{5}}							& $0.480$				& $0.000$					& 
%$0.000$	\\ \midrule
%	   \bfsat{1}~\cite{kasneci2009star} 		& $0.000$				& 
%$0.000$					& $0.000$	\\ 
%	   \bfsat{3} 		& $0.000$				& $0.000$					& $0.000$	\\ 
%	   \bfsat{5} 		& $0.000$				& $0.000$					& $0.000$	\\ 
%\midrule
%       \paralex~\cite{fader2013paraphrase} 	& $0.000$				& 
%$0.000$					& $0.000$	\\ 
%       \paralex+Auto Decomp. 				& $0.000$				& $0.000$					
%& $0.000$	\\
%       \paralex+Manual Decomp. 				& $0.000$				& 
%$0.000$					& $0.000$	\\ 
%\midrule
%       \aqqu~\cite{bast2015more} 			& $0.000$				& 
%$0.000$					& $0.000$	\\
%       \aqqu+Auto Decomp. 					& $0.000$				& $0.000$					& 
%$0.000$	\\
%       \aqqu+Man. Decomp.+Rel. Union 		& $0.000$				& 
%$0.000$					& $0.000$	\\ 
%       \bottomrule            
%    \end{tabular}

==> tbl-oie-examples.tex <==
{
\begin{tabular}{p{8cm}}
       \toprule
       \textbf{Input Sentence}: 
       Samuel Umtiti, born 14 November 1993, in Yaounde, Cameroon, is a French
       professional footballer who plays as a centre-back for Spanish club
       Barcelona and is a member of the France national team.  \\ \toprule
       \textbf{Stanford OpenIE v3.7}~\cite{angeli2015leveraging}:
       (Samuel Umtiti, born, 14 November 1993),
       (Samuel Umtiti, in, Yaounde),
       (Umtiti, is, French),
       (Umtiti, is, professional) \\ \midrule
       \textbf{OpenIE v4.3}~\cite{mausam2016open}: \textcolor{red}{to-do}\\ \midrule
       \textbf{ClausIE}~\cite{del2013clausie}:
       (Samuel Umtiti, be born, 14 November 1993 in Yaounde Cameroon),
       (Samuel Umtiti, be born, 14 November 1993),
       (Samuel Umtiti born 14 November 1993 in Yaounde Cameroon, is, a French
       professional footballer),
       (a French professional footballer, plays, as a centre-back for Spanish
       club Barcelona),
       (a French professional footballer, is, a member of the France national
       team),
       (a French professional footballer, is, a member) \\ \midrule
       \textbf{{\quest}'s Noisy OpenIE}: \textcolor{red}{to-do}\\ \bottomrule   
    \end{tabular} %}
}%\footnotesize
%{\footnotesize
%\begin{tabular}{p{3.5cm} p{14cm}}
%       \toprule
%       \textbf{Input Sentence} 											& Didier Yves Drogba T\'{e}bily (born 11 March 1978) is 
%       an Ivorian professional footballer who plays as a striker for American club Phoenix Rising. \\ \toprule
%       \textbf{Stanford OpenIE v3.7}~\cite{angeli2015leveraging} 	& (T\'{e}bily, is, Ivorian), (T\'{e}bily, is, 
%       professional), (Phoenix Rising, for, American) \\ \midrule
%       \textbf{OpenIE v4.3}~\cite{mausam2016open}					& (Didier Yves Drogba T\'{e}bily born 11 
%       March 1978, is, an Ivorian professional footballer who plays as a
%																       striker for American club Phoenix Rising), (an Ivorian 
%																       professional footballer, plays, NULL)				\\ \midrule
%       \textbf{ClausIE}~\cite{del2013clausie}						& (Didier Yves Drogba T\'{e}bily born 11 March 
%       1978, is, an Ivorian professional footballer),
%																       (an Ivorian professional footballer, plays, as a striker for 
%																       American club Phoenix Rising)			\\ \midrule
%       \textbf{{\quest}'s noisy OpenIE}						& (Didier Yves Drogba T\'{e}bily, born, 11 March 
%       1978),
%																       (Didier Yves Drogba T\'{e}bily, born, Ivorian),
%																       (Didier Yves Drogba T\'{e}bily, born, footballer),
%																       (Didier Yves Drogba T\'{e}bily, born, striker),
%																       (Didier Yves Drogba T\'{e}bily, born, American),
%																       (Didier Yves Drogba T\'{e}bily, born, Phoenix Rising),
%																       (Ivorian, plays, striker),
%																       (Ivorian, plays, American),
%																       (Ivorian, plays, Phoenix Rising),
%																       (footballer, plays, striker),
%																       (footballer, plays, American),
%																       (footballer, plays, Phoenix Rising)\\ \bottomrule   
%    \end{tabular} %}
%}%\footnotesize

==> tbl-ranking-intuition-comparisons.tex <==
\begin{tabular}{l c c}
   \toprule
	\textbf{Answer ranking criterion}		&	\textbf{CQ-150}			&	\textbf{TQ-100}			\\ \toprule
	Sum of node weights						&	$\boldsymbol{0.315}$	&	$\boldsymbol{0.351}$	\\ \midrule
	Number of GSTs ($k$)					&	$0.314$					&	$0.347$	\\
	Sum of inverses of tree costs			&	$0.306$					&	$0.344$					\\ 
	Weighted distance to all cornerstones	&	$0.252$*				&	$0.281$*				\\
	Unweighted distance to all cornerstones	&	$0.270$*				&	$0.291$*				\\ \bottomrule
\end{tabular}

==> tbl-resources.tex <==
 \begin{tabular}{l c c}
       \toprule
		\textbf{Resources used}	& 	\textbf{CQ-150}		& 	\textbf{TQ-150}		\\ \toprule
		Both					& 	$0.317$					& 	$0.267$					\\ \midrule
		No AIDA	lexicon			& 	$0.322$					& 	$0.289$					\\
		No \method{GloVe}		& 	$0.328$					& 	$\boldsymbol{0.303}$	\\
		None					& 	$\boldsymbol{0.333}$	& 	$0.282$					\\ \bottomrule
    \end{tabular} 
